Diamonds are Forever in the Blockchain: Geometric Polyhedral Point-Set Pattern Matching

Motivated by blockchain technology for supply-chain tracing of ethically sourced diamonds, we study geometric polyhedral point-set pattern matching as minimum-width polyhedral annulus problems under translations and rotations. We provide two $(1 + \varepsilon)$-approximation schemes under translations with $O(\varepsilon^{-d} n)$-time for $d$ dimensions and $O(n\log \varepsilon^{-1} + \varepsilon^{-2})$-time for two dimensions, and we give an $O(f^{d-1}\varepsilon^{1-2d}n)$-time algorithm when also allowing for rotations, parameterized on $f$, which we define as the slimness of the point set.

==> expandedprelim.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\begin{definition}
Following previous
convention~\cite{amenta2007size,attali2003complexity,attali2004linear,erickson2001nice,amenta1999surface},
we say that
a point set~$S$ is a
\emph{$\delta$-uniform sample} of a surface $\Sigma \subset \mathbb{R}^d$
if for every point $p \in \Sigma$, there exists a point $q \in S$ such that
$d(p, q) \leq \delta$.
\end{definition}
\begin{definition}
Let $C \subset \mathbb{R}^d$ be a polyhedron containing the origin. Given $C$, and $x \in \mathbb{R}^d$, define $x + C = \{x + y : y \in C\}$ (the translation of~$C$ by~$x$), and for $r \in \mathbb{R}$, define $r C = \{r y : y \in C\}$. A \emph{placement} of $C$ is a pair $(x,r)$, where $x \in \mathbb{R}^d$ and $r \in \mathbb{R}^{\geq 0}$, representing the translated and scaled copy $x + r C$. We refer to $x$ and $r$ as the \emph{center} and \emph{radius} of the placement, respectively. Two placements are \emph{concentric} if they share the same center.
\end{definition}
\begin{definition}
Let $C$ be any closed convex body in  $\mathbb{R}^d$ containing the origin in its interior. The convex distance function induced by $C$ is the function $d_C: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}^{\geq 0}$, where $d_C(p,q) = \min \{r : r \geq 0 ~\mathrm{and}~ q \in p + r C\}$.
Thus, the convex distance between $p$ and $q$ is determined by the minimum radius placement of $C$ centered at $p$ that contains $q$ (see Figure~\ref{fig:prelims}). When $C$ is centrally symmetric, this defines a metric, but for general $C$, the function $d_C$ may not be symmetric. We call the original shape $C$ the \emph{unit ball} $U_C$ under the distance function $d_C$.
Note that $d_C(a,c)= d_C(a,b)+d_C(b,c)$ when $a$, $b$ and $c$ are colinear and appear in that order.
\end{definition}

\begin{definition}
\label{def:annulus}
Define an \emph{annulus} for $C$ to be the set-theoretic difference of two concentric placements $(p + R C) \setminus (p + r C)$, for $0 \leq r \leq R$. The \emph{width} of the annulus is $R - r$.
\end{definition}
Given a $\delta$-uniform sample of points, $S$, 
there are three placements of $C$ we are interested in:
\begin{definition}
\label{def:MinBall}
\textbf{Minimum enclosing ball (MinBall)}:  A placement of $C$ of the smallest radius that contains all of the points in $S$. 
\end{definition}
\begin{definition}
\label{def:MaxBall}
\textbf{Maximum enclosed ball (MaxBall)}: A placement of $C$ of the largest radius, centered within the convex hull of $S$, that contains no points in~$S$.
\end{definition}
\begin{definition}
\label{def:MWA}
\textbf{Minimum width annulus (MWA)}: Given a set $S \subset \mathbb{R}^d$ and a convex body $C$, the minimum width annulus of $S$ is the annulus for $C$ of the smallest width that contains $S$. 
\end{definition}
Note that, following the definition of the MaxBall in \Cref{def:MaxBall},
we require that
the center of the MWA must also lie within the convex hull of $S$.
For each of the above placements, we also refer to parameterized versions, for example MinBall($p$), MaxBall($p$), or MWA($p$). 
These respectively refer to the minimum enclosing ball, maximum enclosed ball, or minimum width annulus {centered at the point $p$}.

Further, we use $|\MinBall(p)|$ and $|\MaxBall(p)|$ to 
denote the radius of MinBall$(p)$ and MaxBall$(p)$, respectively, 
and we use $|\MWA(p)|$ to denote the width of MWA$(p)$.


\begin{definition}
\label{def:fatness}
\emph{Fatness:} The fatness, $F$, of $S\subset\mathbb{R}^d$ under $d_C$ as the ratio of the \MinBall\ over the \MaxBall, such that $F:=|\MinBall|/|\MaxBall|$. Note that $S$ can either be a closed body in $\mathbb{R}^d$ or sample of a surface.
\end{definition}
\begin{definition}
\emph{Concentric Fatness:} Extend the notion of fatness such that the concentric fatness, $F_c:=|\MinBall(c)|/|\MaxBall(c)|$ such that $c$ is the center of the MWA.
\end{definition}
\begin{definition}
\emph{Slimness:} Conversely to concentric fatness, define the slimness, $f$, as the ratio of the width of the \MWA\ centered at $c$ over the radius of \MinBall(c), such that $f:=|\MinBall(c)|/|\MWA|$ and $f^{-1}=1-F_c^{-1}$.
\end{definition}
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{img/distfnprelims}
    \caption{\textbf{Left:} a visual representation of a polyhedral distance function and the distance between two points. \textbf{Center:} The MinBall under $d_C$ containing all points in $S$, centered at $c$. \textbf{Right:} The MWA of $S$ with all points within MinBall$(c)\setminus $MaxBall(c).}
    \label{fig:prelims}
\end{figure}

\begin{remark} 
\label{rm:deltauniformity}
In order for a $\delta$-uniform sample to represent the surface, $\Sigma$, with enough accuracy for a meaningful $\MWA$, the sample must contain at least one point between corresponding facets of the $\MWA$. Where corresponding facets refer to facets of the \MinBall\ and \MaxBall\ representing the same facet of $U_C$. Therefore, 
in the remainder of the chapter, we assume we have a $\delta$-uniform sample and 
that $\delta$ is small enough to guarantee this condition for even the smallest facets. 
\end{remark}

In practice, it would be easy to determine a small enough $\delta$ before sampling $\Sigma$, since only sufficiently slim surfaces would benefit from finding the $\MWA$ and very fat surfaces would yield increasingly noisy $\MaxBall$. Thus, setting $\delta$ to the smallest facet of the $\MinBall$ and scaling down by an arbitrary constant larger than the maximum expected fatness, such as 100, will easily yield a small enough $\delta$.

Also, note that, for a center point $c$, 
the problem of finding $\MWA(c)$
has a unique solution, because a unit ball, $U_C$, is 
convex and once the placement's radius grows past $d_C(c,p)$,
it must contain $p\in S$. Thus, the inner and outer radii are defined as $\min_{p\in S}  d_C(c,p)$ and $\max_{p\in S} d_C(c,p)$, respectively. 
Further, let us assume
that the reference polytope defining our polyhedral distance function
has $m$ facets, where $m$ is a fixed constant,
since the sample size is expected to be 
much larger than $m$. Thus,
$\dc$ can be calculated in $O(m)$ time; hence, $\MWA(c)$ can be 
found in $O(mn)$ time, which is $O(n)$ under a fixed polytope. 


